UltraRAG: A Modular and Automated Toolkit for Adaptive Retrieval-Augmented Generation

Retrieval-Augmented Generation (RAG) significantly enhances the performance of large language models (LLMs) in downstream tasks by integrating external knowledge. To facilitate researchers in deploying RAG systems, various RAG toolkits have been introduced. However, many existing RAG toolkits lack support for knowledge adaptation tailored to specific application scenarios. To address this limitation, we propose UltraRAG, a RAG toolkit that automates knowledge adaptation throughout the entire workflow, from data construction and training to evaluation, while ensuring ease of use. UltraRAG features a user-friendly WebUI that streamlines the RAG process, allowing users to build and optimize systems without coding expertise. It supports multimodal input and provides comprehensive tools for managing the knowledge base. With its highly modular architecture, UltraRAG delivers an end-to-end development solution, enabling seamless knowledge adaptation across diverse user scenarios. The code, demonstration videos, and installable package for UltraRAG are publicly available at https://github.com/OpenBMB/UltraRAG.

==> latex/4.5_discussion.tex <==
\section{Discussion and Future Work}
In this section, we outline our plans for future work. Moving forward, we aim to further enhance the adaptability and performance of the framework, with a particular focus on the following areas:

\textbf{Incorporating Advanced RAG Algorithms.} We intend to continuously integrate more advanced RAG algorithms, striving to build an all-in-one platform that simplifies the process of reproducing research for researchers. Our goal is to make it easier for researchers to reproduce existing algorithms while also encouraging contributions from the open-source community.

\textbf{Optimizing the Framework.} We will continue to improve the WebUI to better meet the diverse needs of users. For novice users, we plan to provide a one-click deployment feature, enabling them to train and deploy RAG applications without dealing with the underlying complexities. For more advanced users, we will introduce additional customizable options, allowing them to better compare and evaluate different RAG algorithms. Furthermore, we will work on creating a more intuitive RAG pipeline, offering a visual interface for input-output management at each stage and incorporating drag-and-drop functionality to simplify the user experience.




==> table/evaluation.tex <==
\begin{table}[ht]
% \begin{table*}[ht]
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{lccc}
\hline
\multicolumn{4}{c}{\textbf{Retrieval Performance}} \\
\hline
\textbf{Method} & \textbf{MRR@10} & \textbf{NDCG@10} & \textbf{Recall@10} \\
\hline
Finetune & 37.57 & 42.12 & 56.50 \\
\ \ \ \textit{w/o} Finetune & 36.46 & 40.05 & 54.50 \\
\end{tabular}}
\hfill
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{lc|lc}
\hline
\multicolumn{2}{c|}{\textbf{Law Prediction (3-2)}} & \multicolumn{2}{c}{\textbf{Consultation (3-8)}} \\
\hline
\textbf{Method} & \textbf{ROUGE-L} & \textbf{Method} & \textbf{ROUGE-L} \\
\hline
VanillaRAG & 40.75 & VanillaRAG & 23.65 \\
KBAlign & 48.72 & DeepNote & 24.62 \\
RAG-DDR & 53.14& Finetune & 25.85 \\
\hline
\end{tabular}}

\caption{Evaluation Results of Retrieval and Generation Performance.}
\label{tab:side_by_side_results}
% \end{table*}
\end{table}


